Particip-AI: A Democratic Surveying Framework for Anticipating Future AI Use Cases, Harms and Benefits

General purpose AI, such as ChatGPT, seems to have lowered the barriers for the public to use AI and harness its power. However, the governance and development of AI still remain in the hands of a few, and the pace of development is accelerating without a comprehensive assessment of risks. As a first step towards democratic risk assessment and design of general purpose AI, we introduce PARTICIP-AI, a carefully designed framework for laypeople to speculate and assess AI use cases and their impacts. Our framework allows us to study more nuanced and detailed public opinions on AI through collecting use cases, surfacing diverse harms through risk assessment under alternate scenarios (i.e., developing and not developing a use case), and illuminating tensions over AI development through making a concluding choice on its development. To showcase the promise of our framework towards informing democratic AI development, we run a medium-scale study with inputs from 295 demographically diverse participants. Our analyses show that participants' responses emphasize applications for personal life and society, contrasting with most current AI development's business focus. We also surface diverse set of envisioned harms such as distrust in AI and institutions, complementary to those defined by experts. Furthermore, we found that perceived impact of not developing use cases significantly predicted participants' judgements of whether AI use cases should be developed, and highlighted lay users' concerns of techno-solutionism. We conclude with a discussion on how frameworks like PARTICIP-AI can further guide democratic AI development and governance.

==> content/figures/usecase-count-figure.tex <==
\begin{figure*}[htpb]
  \centering
  \subcaptionbox{Q7\label{subfig:use-case-themes}}{%
     \includegraphics[width=0.4\textwidth]{content/figures/Q7_4-theme-percentage-graph-0107v1.pdf}%
  }\hfill
  \subcaptionbox{\label{subfig:use-case-codes}}{%
    \includegraphics[width=0.55\textwidth]{content/figures/Q7_4-code-percentage-graph-0107v1.pdf}
  }
  \subcaptionbox{Q3\label{subfig:use-case-themes}}{%
     \includegraphics[width=0.4\textwidth]{content/figures/Q3-theme-percentage-graph-0107v1.pdf}%
  }\hfill
  \subcaptionbox{\label{subfig:use-case-codes}}{%
    \includegraphics[width=0.55\textwidth]{content/figures/Q3-code-percentage-graph-0107v1.pdf}
  }
  \subcaptionbox{Q6\label{subfig:use-case-themes}}{%
     \includegraphics[width=0.4\textwidth]{content/figures/Q6-theme-percentage-graph-0107v1.pdf}%
  }\hfill
  \subcaptionbox{\label{subfig:use-case-codes}}{%
    \includegraphics[width=0.55\textwidth]{content/figures/Q6-code-percentage-graph-0107v1.pdf}
  }
  \caption{Use Cases}
  \label{fig:use-cases}
\end{figure*}

==> content/tables-old/Q11-Q14-table.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.23\linewidth}|p{0.70\linewidth}|p{0.05\linewidth}p{0.05\linewidth}}
    \toprule
        & & \multicolumn{2}{c}{\textbf{\% responses}} \\
        \textbf{Code} & \textbf{Quote \& Scale of Impact (Q13 / Q16)} & \hfil \textbf{Q11} & \hfil \textbf{Q14} \\
        & & \hfil $295\times$ & \hfil $295\times$ \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Social \& psychological effect}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.82$\pm$1.94 / 5.29$\pm$2.05} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{35.3\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{26.4\%} \\
        \hline
        \texttt{Manipulate people} &  \textit{``People would lose control potentially over important data, ideas...''} (P113, Q11) & \hfil 12.9\% & \hfil 1.0\% \\
        \texttt{Misinformation} & \hangindent=1em \textit{``It could give false information and confuse people as to where they don’t know which source of information to trust"} (P126, Q11) & \hfil 12.5\% & \hfil 10.8\% \\
        \texttt{Mental harm} & \hangindent=1em \textit{``Loss of confidence and motivation: Repeated misunderstandings and failed interactions could lead to frustration and a reluctance to engage in...learning.''} (P280, Q14) & \hfil 12.2\% & \hfil 9.5\% \\
        \texttt{Social isolation} & \textit{``It would harm...relationships...maybe [leading] to ostracism or loss of trust.''} (P200, Q14) & \hfil 2.4\% & \hfil 4.4\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Economic impact}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.39$\pm$1.70 / 4.63$\pm$1.75} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{32.5\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{33.6\%} \\
        \hline
        \texttt{Financial disturbance} &  \textit{``People would lose jobs and incomes''} (P93, Q11) & \hfil 16.3\% & \hfil 20.7\% \\
        \texttt{Economic disturbance} & \textit{``Shortage in suppliers or a raise in costs"} (P126, Q11) & \hfil 12.9\% & \hfil 9.8\% \\
        \texttt{Waste resources or time} & \textit{``Potentially leading to misguided decisions [and] wasted resources...''} (P250, Q14) & \hfil 1.0\% & \hfil 9.5\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Safety \& security risk}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.32$\pm$1.57 / 6.10$\pm$1.60} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{21.7\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{7.8\%} \\
        \hline
        \texttt{Data security \& privacy risk} & \textit{``It could be...compromising users' private data''} (P235, Q14) & \hfil 10.5\% & \hfil 3.1\% \\
        \texttt{Extinction} & \textit{``human race eliminated by machines''} (P220, Q11) & \hfil 5.8\% & \hfil 2.0\% \\
        \texttt{Aid criminal} & \textit{``It will lead to theft''} (P275, Q14) & \hfil 4.1\% & \hfil 2.7\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Physical effect}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.70$\pm$1.40 / 6.28$\pm$1.59} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{16.9\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{29.8\%} \\
        \hline
        \texttt{Physical harm} &  \textit{``It could lead to serious injury  or death.''} (P215, Q14) & \hfil 12.9\% & \hfil 23.7\% \\
        \texttt{Negative health \& well-being} & \textit{``People would become more unhealthy''} (P175, Q11) & \hfil 3.4\% & \hfil 8.5\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Quality \& reliability issues of AI}}\hspace{93pt}\textbf{5.16$\pm$1.76 / 5.43$\pm$2.12}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{15.9\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{24.1\%} \\
        \hline
        \texttt{Incorrect AI output} &\textit{``Providing incorrect or incomplete medical diagnostics''} (P221, Q14) & \hfil 9.8\% & \hfil 13.6\% \\
        \texttt{Distrust AI} & \textit{``People would lose trust in technology''} (P72, Q11) & \hfil 5.1\% & \hfil 5.8\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Impeding human development \& learning}}\hspace{66pt}\textbf{4.41$\pm$1.80 / 4.42$\pm$2.10}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{12.9\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{12.5\%} \\
        \hline
        \texttt{Overreliance} & \textit{``[People] will not learn to do anything on their own''} (P274, Q14) & \hfil 9.5\% & \hfil 6.8\% \\
        \texttt{Impede learning} &\textit{``Diminished capacity for original ideas, maybe even critical thinking''} (P221, Q11) & \hfil 3.7\% & \hfil 3.7\% \\
        \texttt{Hinder career} & \textit{``The reputation of the developers would be ruined''} (P125, Q14) & \hfil 1.0\% & \hfil 4.1\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Reducing quality \& reliability of society}}\hspace{64pt}\textbf{5.70$\pm$2.01 / 5.48$\pm$2.09}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{12.2\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{9.2\%} \\
        \hline
        \texttt{Distrust institution} & \textit{``The negative impact would be...decreased trust in the medical professionals...''} (P62, Q14) & \hfil 5.8\% & \hfil 5.4\% \\
        \texttt{Legal issues} & \textit{``Increased lawsuits.''} (P95, Q14) & \hfil 3.1\% & \hfil 4.1\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{General harm}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.95$\pm$2.25 / 5.97$\pm$1.94} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.8\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{11.5\%} \\
        \hline
        \texttt{General harm} & \textit{``More people would be hurt''} (P105, Q11) & \hfil 4.7\% & \hfil 10.2\% \\
        \texttt{Range} & \textit{``Could cause anything from minor issues to loss of life''} (P271, Q14) & \hfil 2.0\% & \hfil 1.7\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Reducing progress}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{7.50$\pm$0.84 / 6.57$\pm$1.45} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{2.0\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{4.7\%} \\
        \hline
        \texttt{Environmental harm} & \textit{``It could negatively impact fighting climate change''} (P23, Q14) & \hfil 1.4\% & \hfil 1.7\% \\
        \texttt{Hinder science} &  \textit{``Delay scientific advancement and progress''} (P276, Q14) & \hfil 0.7\% & \hfil 3.1\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Other}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{3.30$\pm$3.22 / 4.28$\pm$2.83} &  \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{4.4\%} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{7.1\%} \\
        \hline
        \texttt{N/A} & \textit{``Many things''} (P216, Q11) & \hfil 2.4\% & \hfil 2.7\% \\
        \texttt{No harm} & \textit{``I can't think of any [harms]''} (P242, Q11) & \hfil 1.7\% & \hfil 3.7\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Harms of developing (Q11, Q14): percentage of occurrence for \textsc{theme} with scale of impact (Q13, Q16) and corresponding top few most frequent \texttt{codes} with representative quotes.}
    \label{tab:q11-theme}
\end{table*}

==> content/tables-old/Q11-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q11 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{social and psychological effect}} & \multirow{3}{*}{35.3} & \texttt{manipulate-people} & 36.5 & \textit{``People would lose control potentially over important data, ideas, ...''} (P113)\\
         &  & \texttt{misinformation} & 35.6 & \textit{``It could give false information and confuse people as to where they don't know which source of information to trust''} (P126)\\
         &  & \texttt{mental-harm} & 34.6 & \textit{``People wanting to commit suicide maybe...''} (P67)\\
         \hline
        \multirow{2}{*}{\textsc{economic impact}} & \multirow{2}{*}{32.5} & \texttt{financial-disturbance} & 50 & \textit{``People would lose jobs and incomes''} (P93)\\
         &  & \texttt{economic-disturbance} & 39.6 & \textit{``Shortage in suppliers or a raise in costs''} (P131)\\
         \hline
        \multirow{2}{*}{\textsc{safety and security risk}} & \multirow{2}{*}{21.7} & \texttt{data-security-privacy-risk} & 48.4 & \textit{``Breach in privacy...''} (P179)\\
         &  & \texttt{extinction} & 26.6 & \textit{``human race eliminated by machines''} (P220)\\
         \hline
        \multirow{2}{*}{\textsc{physical effect}} & \multirow{2}{*}{16.9} & \texttt{physical-harm} & 76 & \textit{``Someone might fall very ill or even die''} (P246)\\
         &  & \texttt{negative-health-wellbeing} & 20 & \textit{``people would become more unhealthy''} (P175)\\
         \hline
        \multirow{2}{*}{\textsc{quality and reliability issues of AI}} & \multirow{2}{*}{15.9} & \texttt{incorrect-ai-output} & 61.7 & \textit{``people might be misdiagnosed and take action based on that''} (P264)\\
         &  & \texttt{distrust-ai} & 31.9 & \textit{``People would lose trust in technology''} (P72)\\
         \hline
        \multirow{2}{*}{\textsc{impeding human development and learning}} & \multirow{2}{*}{12.9} & \texttt{overreliance} & 73.7 & \textit{``it could steer people into a cult like dependency on AI as a blindly trusted leader.''} (P88)\\
         &  & \texttt{impede-learning} & 28.9 & \textit{``Diminished capacity for original ideas, maybe even critical thinking''} (P221)\\
         \hline
        \multirow{2}{*}{\textsc{reducing quality and reliability of society}} & \multirow{2}{*}{12.2} & \texttt{distrust-institution} & 47.2 & \textit{``If widespread, it could cause a financial meltdown and a complete lack of trust in companies. ''} (P255)\\
         &  & \texttt{legal-issues} & 25 & \textit{``possible biological agents or increased lawsuits.''} (P95)\\
         \hline
        \multirow{2}{*}{\textsc{general harm}} & \multirow{2}{*}{6.8} & \texttt{general-harm} & 70 & \textit{``More people would be hurt''} (P105)\\
         &  & \texttt{range} & 30 & \textit{``A select few suffering more than others.''} (P108)\\
         \hline
        \multirow{2}{*}{\textsc{other}} & \multirow{2}{*}{4.4} & \texttt{na} & 53.8 & \textit{``many things''} (P216)\\
         &  & \texttt{no-harm} & 38.5 & \textit{``I can’t think of any''} (P242)\\
         \hline
        \multirow{2}{*}{\textsc{reducing progress}} & \multirow{2}{*}{2.0} & \texttt{environmental-harm} & 66.7 & \textit{``Climate change could be made even worse.''} (P140)\\
         &  & \texttt{hinder-science} & 33.3 & \textit{``It will destroy the integrity of scientific advancements''} (P276)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q11-theme}
\end{table*}

==> content/tables-old/Q14-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q14 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{economic impact}} & \multirow{2}{*}{33.6} & \texttt{financial-disturbance} & 61.6 & \textit{``Money wasted.''} (P8)\\
         &  & \texttt{economic-disturbance} & 29.3 & \textit{``impoverising the poor more.''} (P54)\\
         &  & \texttt{waste-resources-or-time} & 28.3 & \textit{``potentially leading to misguided decisions, wasted resources, and exacerbation of existing problems.''} (P250)\\
        \hline
        \multirow{2}{*}{\textsc{physical effect}} & 29.8 & \texttt{physical-harm} & 79.5 & \textit{``It could lead to serious injury  or death.''} (P215)\\
         &  & \texttt{negative-health-wellbeing} & 28.4 & \textit{``Poorer health''} (P242)\\
        \hline
        \multirow{2}{*}{\textsc{social and psychological effect}} & 26.4 & \texttt{misinformation} & 41 & \textit{``Action would be taken on invalid info with potential harm''} (P244)\\
         &  & \texttt{mental-harm} & 35.9 & \textit{``Loss of confidence and motivation: Repeated misunderstandings and failed interactions could lead to frustration and a reluctance to engage in further language learning.''} (P280)\\
         &  & \texttt{social-isolation} & 16.7 & \textit{``It would harm social relationships. Not necessarily ending them, but maybe lead to ostracism or loss of trust.''} (P200)\\
        \hline
        \multirow{2}{*}{\textsc{quality and reliability issues of AI}} & 24.1 & \texttt{incorrect-ai-output} & 56.3 & \textit{``It depends on the situation, but for example, providing incorrect or incomplete medical diagnostics''} (P221)\\
         &  & \texttt{distrust-ai} & 23.9 & \textit{``People would start protesting and would try to ban this AI.''} (P50)\\
        \hline
        \multirow{2}{*}{\textsc{impeding human development and learning}} & 12.5 & \texttt{overreliance} & 54.1 & \textit{``They will not learn to do anything on their own''} (P274)\\
         &  & \texttt{hinder-career} & 32.4 & \textit{``The reputation of the developers would be ruined''} (P125)\\
        \hline
        \multirow{2}{*}{\textsc{general harm}} & 11.5 & \texttt{general-harm} & 88.2 & \textit{``I think providing incorrect information could generally just make people's lives harder.''} (P166)\\
         &  & \texttt{range} & 14.7 & \textit{``Could cause anything from minor issues to loss of life''} (P271)\\
        \hline
        \multirow{2}{*}{\textsc{reducing quality and reliability of society}} & 9.2 & \texttt{distrust-institution} & 59.3 & \textit{``The negative impact would be loss of business and decreased trust in the medical professionals...''} (P)\\
         &  & \texttt{legal-issues} & 44.4 & \textit{``It would lead to injuries and potential legal issues.''} (P41)\\
        \hline
        \multirow{2}{*}{\textsc{safety and security risk}} & 7.8 & \texttt{data-security-privacy-risk} & 39.1 & \textit{``It could be anything from software failure to compromising users private data''} (P235)\\
         &  & \texttt{aid-criminal} & 34.8 & \textit{``It will lead to theft''} (P275)\\
        \hline
      \textsc{other} & 7.1 & \texttt{no-harm} & 52.4 & \textit{``none''} (P)\\
        \hline
        \multirow{2}{*}{\textsc{reducing progress}} & 4.7 & \texttt{hinder-science} & 64.3 & \textit{``Delay scientific advancement and progress''} (P276)\\
         &  & \texttt{environmental-harm} & 35.7 & \textit{``it could negatively impact fighting climate change''} (P23)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q14-theme}
\end{table*}

==> content/tables-old/Q17-table.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.2\linewidth}|p{0.74\linewidth}|p{0.1\linewidth}}
    \toprule
        & & \hfil \textbf{\% responses} \\
        \textbf{Code} & \textbf{Quote \& Scale of Impact (Q19)} & \hfil \textbf{Q17} \\
        & & \hfil $295\times$ \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Limiting human potential}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.56$\pm$2.12} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{32.9\%} \\
        \hline
        \texttt{Waste resources or time} &  \textit{``I waste so much time on these types of activities. Time that could be spent on productive things...''} (P39) & \hfil 13.2\% \\
        \texttt{Inefficiency} & \hangindent=1em \textit{``Government and public agencies will continue to operate in a wasteful and ineffective manner.''} (P76) & \hfil 12.2\% \\
        \texttt{Impede personal growth} & \textit{``People would not be able to reach their potentials.''} (P106) & \hfil 11.9\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Lose information \& accessibility to resources}}\hspace{105pt}\textbf{4.14$\pm$2.04}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{26.1\%} \\
        \hline
        \texttt{Lose assistance} & \textit{``Immigrants would not recieve [sic] translation support easily.''} (P122) & \hfil 11.5\% \\
        \hangindent=1em \texttt{Lose solution or service} & \textit{``Homeless need easier more accessible help...''} (P206) & \hfil 9.8\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Other}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{2.73$\pm$2.59} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{23.4\%} \\
        \hline
        \texttt{No harm} & \textit{``It wouldnt [sic] necessarily be harmful''} (P216) & \hfil 16.6\% \\
        \texttt{New code} & \textit{``It may be an emergency''} (P1) & \hfil 4.1\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Less innovation}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{4.64$\pm$2.08} &  \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{15.9\%} \\
        \hline
        \texttt{Delay in innovation} & \textit{``It could slow down progress against climate change''} (P23) & \hfil 9.5\% \\
        \texttt{Less innovation} & \textit{``New technology would not be used to help man kind.''} (P87) & \hfil 8.5\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Social \& psychological effect}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{4.07$\pm$2.40} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{15.6.5\%} \\
        \hline
        \texttt{Stress \& overworked} & \textit{``It would increase the workload and time spent on tedious tasks.''} (P181) & \hfil 10.8\% \\
        \texttt{Mental harm} &  \textit{``It would deprive people of an opportunity to address their loneliness''} (P96) & \hfil 4.7\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Less progress in solving societal issues}}\hspace{145pt}\textbf{4.78$\pm$2.19}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{13.9.5\%} \\
        \hline
        \texttt{Hinder medical care} & \textit{``Many individuals will continue suffering from ailments that...worsen in time.''} (P117) & \hfil 8.5\% \\
        \texttt{Misinformation} &  \textit{``Some people...find bad answers on the internet that make things worse''} (P246) & \hfil 3.7\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Economic \& business impact}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.70$\pm$2.27} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{11.5.5\%} \\
        \hline
        \texttt{Financial disturbance} &  \textit{``Individuals might lack access to highly personalized and good retirement strategies''} (P292) & \hfil 4.7\% \\
        \texttt{Economic disturbance} & \textit{``Increases cost and reduce employment''} (P16) & \hfil 4.1\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Limited to human capabilities}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{4.39$\pm$1.64} &  \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{9.5\%} \\
        \hline
        \texttt{Human error} &  \textit{``Humans are biased...and often unable to combine various fields of thought.''} (P88) & \hfil 6.8\% \\
        \texttt{Hinder creative work} & \textit{``It could hinder some people's ability to create.''} (P120) & \hfil 2.7\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Physical effect}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{5.14$\pm$2.62} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{8.5\%} \\
        \hline
        \texttt{Physical harm} & \textit{``it could've saved a lot of lives''} (P152) & \hfil 5.8\% \\
        \texttt{Health issues} & \textit{``My health will suffer.''} (P30) & \hfil 3.7\% \\
        \bottomrule
    \end{tabular}}
    \caption{Harms of \textit{not} developing (Q17): percentage of occurrence for \textsc{theme} with scale of impact (Q19) and corresponding top few most frequent \texttt{codes} with representative quotes.}
    \label{tab:q17-theme}
\end{table*}

% \begin{table}[htpb]
%     \centering
%     \footnotesize
%     \begin{tabularx}{\textwidth}{l|c|ll|X}
%     \toprule
%         Theme & \makecell{Q17 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
%         \hline
%         \multirow{3}{*}{\textsc{limiting human potential}} & \multirow{3}{*}{32.9} & \texttt{waste-resources-or-time} & 40.2 & \textit{``I waste so much time on these types of activities. Time that could be spent on productive things...''} (P39)\\
%          & & \texttt{inefficiency} & 37.1 & \textit{``government and public agencies will continue to operate in a wasteful and ineffective manner, failing to provide the services they receive funding for''} (P76)\\
%          & & \texttt{impede-personal-growth} & 36.1 & \textit{``people would not be able to reach their potentials.''} (P106)\\
%         \multirow{2}{*}{\textsc{lose information and accessibility to resources}} & \multirow{2}{*}{26.1} & \texttt{lose-assistance} & 44.2 & \textit{``cause said immigrants would not recieve [sic] translation support easily''} (P122)\\
%          & & \texttt{lose-accessibility-solution-service} & 37.7 & \textit{``Homeless need easier more accessible help...''} (P206)\\
%         \multirow{2}{*}{\textsc{other}} & \multirow{2}{*}{23.4} & \texttt{no-harm} & 71 & \textit{``it wouldnt [sic] necessarily be harmful''} (P216)\\
%          & & \texttt{new-code} & 17.4 & \textit{``It may be an emergency''} (P1)\\
%         \multirow{2}{*}{\textsc{less innovation}} & \multirow{2}{*}{15.9} & \texttt{delay-in-innovation} & 59.6 & \textit{``It could slow down progress against climate change''} (P23)\\
%          & & \texttt{less-innovation} & 53.2 & \textit{``New technology would not be used to help man kind.''} (P87)\\
%         \multirow{2}{*}{\textsc{social and psychological effect}} & \multirow{2}{*}{15.6} & \texttt{stress-overworked} & 69.6 & \textit{``It would increase the workload and time spent on tedious tasks.''} (P181)\\
%          & & \texttt{mental-harm} & 30.4 & \textit{``it would deprive people of an opportunity to address their loneliness''} (P96)\\
%         \multirow{2}{*}{\textsc{less progress in solving societal issues}} & \multirow{2}{*}{13.9} & \texttt{hinder-medical-care} & 61 & \textit{``Many individuals will continue suffering from ailments that could potentially worsen in time.''} (P117)\\
%          & & \texttt{misinformation} & 26.8 & \textit{``some people might not get answers they need or find bad answers on the internet that make things worse''} (P246)\\
%         \multirow{2}{*}{\textsc{economic and business Impact}} & \multirow{2}{*}{11.5} & \texttt{financial-disturbance} & 41.2 & \textit{``individuals might lack access to highly personalized and good retirement strategies''} (P292)\\
%          & & \texttt{economic-disturbance} & 35.3 & \textit{``increases cost and reduce employment''} (P16)\\
%         \multirow{2}{*}{\textsc{limited to human capabilities}} & \multirow{2}{*}{9.5} & \texttt{human-error} & 71.4 & \textit{``humans are biased and limited and often unable to combine various fields of thought.''} (P88)\\
%          & & \texttt{hinder-creative-work} & 28.6 & \textit{``it could hinder some people's ability to create.''} (P120)\\
%         \multirow{2}{*}{\textsc{physical effect}} & \multirow{2}{*}{8.5} & \texttt{physical-harm} & 68 & \textit{``it could've saved a lot of lives''} (P152)\\
%          & & \texttt{health-issues} & 44 & \textit{``My health will suffer.''} (P30)\\
%         \bottomrule
%     \end{tabularx}
%     \caption{Caption}
%     \label{tab:q17-theme}
% \end{table}

==> content/tables-old/Q20-table.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.26\linewidth}|p{0.68\linewidth}|p{0.1\linewidth}}
    \toprule
        & & \hfil \textbf{\% responses} \\
        \textbf{Code} & \textbf{Quote \& Scale of Impact (Q22)} & \hfil \textbf{Q20} \\
        & & \hfil $295\times$ \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Human growth \& potential}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.95$\pm$2.08} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{43.4\%} \\
        \hline
        \texttt{Less dependent on technology} & \hangindent=1em \textit{``People would think critically and rely on the thoughts of other human beings who have a more nuanced understanding of real life situations then AI ever could.''} (P113) & \hfil 26.4\% \\
        \texttt{Learning skills \& knowledge} &  \textit{``It would make it so more people would strive to learn the local language''} (P122) & \hfil 20.7\% \\
        \texttt{Human interaction dependence} &  \textit{``I might have to communicate that I need help and hopefully would bring us together.''} (P249) & \hfil 13.2\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Economic impact / security}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.54$\pm$2.23} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{22.4\%} \\
        \hline
        \texttt{Job security} &  \textit{``It will not take over peoples' jobs.''} (P251) & \hfil 17.6\% \\
        \texttt{Financial benefit} & \hangindent=1em \textit{``The insurance companies and doctors...make more money off of multiple visits''} (P272) & \hfil 6.8\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Other}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.05$\pm$2.79} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{18.6\%} \\
        \hline
        \texttt{No benefit} &  \textit{``I don't see any benefits''} (P272) & \hfil 10.8\% \\
        \texttt{New code} &  \textit{``The company could put in more effort''} (P148) & \hfil 4.4\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Less bad AI usage}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.66$\pm$2.41} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{15.6\%} \\
        \hline
        \texttt{Less improper or unethical use} &  \textit{``It would not allow for the potential harmful uses of the ai assistance''} (P235) & \hfil 9.5\% \\
        \texttt{More privacy} &  \textit{``It would protect information of all and keep breaches at a minimum''} (P293) & \hfil 4.4\% \\
        \hline
        \multicolumn{2}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Increase transparency, control, \& reliability}}\hspace{65pt}\textbf{3.34$\pm$2.06}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{12.5\%} \\
        \hline
        \texttt{More attentive} & \textit{``It could foster more personal involvement...in one’s investment choices''} (P31) & \hfil 7.1\% \\
        \texttt{Human control} & \hangindent=1em \textit{``It allows for more deliberate, controlled, and transparent progress...fostering public trust and the responsible development of technology.''} (P204) & \hfil 4.1\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{No changes}}} & \cellcolor[rgb]{ .921,  .921, .921}\hfil\textbf{3.26$\pm$2.33} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{7.8\%} \\
        \hline
        \texttt{Maintain status quo} & \textit{``There would really be no change in society, it would remain the same''} (P216) & \hfil 5.8\% \\
        \texttt{Other non-AI solutions} & \textit{``Advances in medicine woud still occur with use of other technologies and methods''} (P45) & \hfil 2.0\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Beneficial side effects of not using AI}}\hspace{92pt}\textbf{4.75$\pm$2.71}}  & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{2.7\%} \\
        \hline
        \texttt{Better health} & \textit{``People...[would]...seek qualified medical assistance, which could save their life.''} (P43) & \hfil 2.0\% \\
        \texttt{Environmental} & \textit{``AI requires a lot of energy so not developing it will be good for the environment''} (P209) & \hfil 0.7\% \\
        \bottomrule
    \end{tabular}}
    \caption{Benefits of \textit{not} developing (Q20): percentage of occurrence for \textsc{theme} with scale of impact (Q22) and corresponding top few most frequent \texttt{codes} with representative quotes.}
    \label{tab:q20-theme}
\end{table*}

% \begin{table}[htpb]
%     \centering
%     \footnotesize
%     \begin{tabularx}{\textwidth}{l|c|ll|X}
%     \toprule
%         Theme & \makecell{Q20 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
%         \hline
%         \multirow{3}{*}{\textsc{human growth and potential}} & \multirow{3}{*}{43.4} & \texttt{less-dependent-on-tech} & 60.9 & \textit{``People would think critically and rely on the thoughts of other human beings who have a more nuanced understanding of real life situations then AI ever could.''} (P113)\\
%          & & \texttt{learning-skills-knowledge} & 47.7 & \textit{``cause it would make it so more people would strive to learn the local language''} (P122)\\
%          & & \texttt{human-interaction-dependence} & 30.5 & \textit{``I might have to communicate that I need help and hopefully would bring us together.''} (P249)\\
%         \multirow{2}{*}{\textsc{economic impact / security}} & \multirow{2}{*}{22.4} & \texttt{job-security} & 78.8 & \textit{``it will not take over peoples' jobs.''} (P251)\\
%          & & \texttt{financial-benefit} & 30.3 & \textit{``The insurance companies and doctors will continue to make more money off of multiple visits''} (P272)\\
%         \multirow{2}{*}{\textsc{other}} & \multirow{2}{*}{18.6} & \texttt{no-benefit} & 58.2 & \textit{``I don't see any benefits''} (P272)\\
%          & & \texttt{new-code} & 23.6 & \textit{``The company could put in more effort''} (P148)\\
%         \multirow{2}{*}{\textsc{less bad ai usage}} & \multirow{2}{*}{15.6} & \texttt{less-improper-unethical-use} & 60.9 & \textit{``It would not allow for the potential harmful uses of the ai assistance''} (P235)\\
%          & & \texttt{more-privacy} & 28.3 & \textit{``It would protect information of all and keep breaches at a minimum''} (P293)\\
%         \multirow{2}{*}{\textsc{increase transparency, control, and reliability}} & \multirow{2}{*}{12.5} & \texttt{more-attentive} & 56.8 & \textit{``it would be beneficial because it could foster more personal involvement and responsibility in one's investment choices''} (P31)\\
%          & & \texttt{human-control} & 32.4 & \textit{``... it would be beneficial because it allows for more deliberate, controlled, and transparent progress.. fostering public trust and the responsible development of technology.''} (P204)\\
%         \multirow{2}{*}{\textsc{no changes}} & \multirow{2}{*}{7.8} & \texttt{maintain-status-quo} & 73.9 & \textit{``there would really be no change in society, it would remain the same''} (P216)\\
%          & & \texttt{other-non-ai-solutions} & 26.1 & \textit{``Advances in medicine woud still occur with use of other technologies and methods''} (P45)\\
%         \multirow{2}{*}{\textsc{beneficial side effects of not using ai}} & \multirow{2}{*}{2.7} & \texttt{better-health} & 75.0 & \textit{``people might be forced to seek qualified medical assistance, which could save their life.''} (P43)\\
%          & & \texttt{environmental} & 25.0 & \textit{``AI requires a lot of energy so not developing it will be good for the environment''} (P209)\\
%         \bottomrule
%     \end{tabularx}
%     \caption{Caption}
%     \label{tab:q20-theme}
% \end{table}

==> content/tables-old/Q3-Q6-Q7-table.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{\footnotesize
    \begin{tabular}{p{0.24\linewidth}|p{0.56\linewidth}|p{0.05\linewidth}p{0.05\linewidth}p{0.05\linewidth}}
    \toprule
        & & \multicolumn{3}{l}{\textbf{\hfill \% responses}} \\
        \textbf{\texttt{Code} / \textsc{Theme}} & \textbf{Quote} & \hfil \textbf{Q3} & \hfil \textbf{Q6} & \hfil \textbf{Q7} \\
        & & $1032\times$ & $992\times$ & $295\times$ \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Domain}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{55.0\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{63.2\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{67.8\%} \\
        \hline
        \texttt{Artistic expression} & \textit{``Make abstract art with my dog's picture''} (P13, Q3) & \hfil 13.4\% & \hfil 3.4\% & \hfil 5.4\% \\
        \texttt{Medical} & \textit{``Automating medical research''} (P54, Q6) & \hfil 4.9\% & \hfil 10.5\% & \hfil 13.9\% \\
        \texttt{Education} & \textit{``Teaching me how to code in different languages''} (P104, Q7) & \hfil 11.1\% & \hfil 9.7\% & \hfil 10.5\%  \\
        \texttt{Research} & \textit{``Revolutionize scientific research''} (P203, Q6) & \hfil 3.0\% & \hfil 8.5\% & \hfil 10.5\%  \\
        \texttt{Translation} & \textit{``Translations while traveling''} (P292, Q3) & \hfil 8.0\% & \hfil 1.3\% & \hfil 4.1\%  \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Support type}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{39.0\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{39.3\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{40.7\%} \\
        \hline
        \texttt{Efficient data analysis} & \hangindent=1em \textit{``Assist in personalized medicine by analyzing genetic data, medical histories, and current research...''} (P242, Q6) & \hfil 8.9\% & \hfil 17.4\% & \hfil 19.0\%  \\
        \texttt{Professional consulting service} & \hangindent=1em \emph{``Mental health diagnosis and intervention...since...professionals often gets overwhelmed with their work."} (P203, Q7)  & \hfil 2.1\% & \hfil 6.3\% & \hfil 7.8\% \\
        \texttt{Writing assistance} & \emph{``Adapting resumes to different job postings''} (P146, Q3)  & \hfil 11.5\% & \hfil 3.6\% & \hfil 2.7\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Personal life}}}  & \cellcolor[rgb]{ .921,  .921, .921} \textbf{45.7\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{39.2\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{29.5\%} \\
        \hline
        \texttt{Everyday task automation} & \textit{``Summarizing important email content into a list''} (P293, Q3)  & \hfil 25.4\% & \hfil 22.1\% & \hfil 14.2\% \\
        \texttt{Everyday life assistance} & \hangindent=1em \textit{``Assisting me with planning meal ideas that meet my family's dietary needs...[to] take much weight off my mental plate.''} (P249, Q7)  & \hfil 17.8\% & \hfil 15.6\% & \hfil 13.9\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Goal of the use case}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{26.5\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{25.9\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{33.6\%} \\
        \hline
        \texttt{Personal life productivity} & \textit{``Assisting with managing time spent on activities"} (P100, Q3)  & \hfil 8.8\% & \hfil 6.0\% & \hfil 10.2\% \\
        \texttt{Creativity} & \hangindent=1em \textit{``Creating unique entertainment options that cater to individuals and evolve with them over time''} (P265, Q6) & \hfil 12.4\% & \hfil 4.6\% & \hfil 6.4\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Society}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{0.3\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{8.7\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{9.5\%} \\
        \hline
        \texttt{Societal issues} & \hangindent=1em \textit{``Predictive models that improve health and environment challenges.''} (P28, Q7) & \hfil0.3\% & \hfil 8.7\% & \hfil 9.5\%  \\
        \hline
       \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Work}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{5.2\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{6.8\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{10.8\%} \\
        \hline
        \texttt{Human labor replacement} & \textit{``Replacing humans in customer interaction jobs''} (P282, Q6) & \hfil 0.8\% & \hfil 4.8\% & \hfil 8.1\%  \\
        \texttt{Workplace productivity} & \textit{``Generate job reports that would take human hours''} (P86, Q6) & \hfil 4.5\% & \hfil 2.5\% & \hfil 4.1\%  \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Other}}} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{0.8\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{2.2\%} & \cellcolor[rgb]{ .921,  .921, .921} \textbf{4.4\%} \\
        \hline
        \texttt{New code} & \textit{``Find a way for the AI to destroy its own AI self''} (P25, Q6) & \hfil 0.8\% & \hfil 2.0\% & \hfil 3.7\%  \\
        \bottomrule
    \end{tabular}}
    \caption{Tasks (Q3, Q6, Q7): percentage of occurrence for \textsc{theme} and top few most frequent \texttt{codes} with representative quotes.}
    \label{tab:q3-q6-q7-theme}
\end{table*}

==> content/tables-old/Q3-Q6-quotes.tex <==
\begin{table*}[!htpb]
    \centering
    \footnotesize
    \begin{tabular}{P{0.25\textwidth}p{0.03\textwidth}p{0.03\textwidth}p{0.59\textwidth}}
    \toprule
    \belowrulesepcolor{cellgray}
    \multicolumn{4}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\emph{Personal life applications}}}\\
    \hline
    \texttt{Search} & Q3 & P245 & ``\textit{Finding specific recipes with specific ingredients}''\\
    % & & P253 & ``\textit{Find the easiest and flattest trails in my area}''\\
    % & Q6 & P52 & ``\textit{Checking for cheaper alternatives to products at different stores}''\\
    % & & Q3 & P82 & ``\textit{Help writing emails using any native language and in a personal style}''\\
    \texttt{Feedback} & Q3 & P107 & ``\textit{Providing ideas on how to improve in certain hobbies}''\\
    & & P46 & ``\textit{Advising on how to discuss sexuality with family without angering them or turning the conversation into an argument}''\\
    % & Q6 & P235 & ``\textit{Analyzing daily jobs and providing time management advice}''\\
    \texttt{Simplification} & Q3 & P210 & ``\textit{Helping people understand complex information related to healthcare, such as doctor's forms/letters, health insurance forms, taxes, etc.}''\\
    \texttt{Efficient data analysis} & Q6 & P75 & ``\textit{Help with resource allocation that maximizes benefit for utilities and food}''\\
    % & & P245 & ``\textit{Analyze personal choices over the past decades and provide recommendations for making better choices about certain things}''\\
    \texttt{Writing assistance} & & P51 & ``\textit{Writing a CV/resume that tailors the job description}''\\
    % & Q3 & P24 & ``\textit{Aiding with time management skills}''\\
    \texttt{Health} & Q3 & P14 & ``\textit{Creating an exercise routine}''\\
    & Q6 & P87 & ``\textit{Replace doctor visits for non-life-threatening ailments}''\\
    \texttt{Mental health} & Q6 & P143 & ``\textit{Monitoring health data and providing personalized insights and recommendations for maintaining physical and mental health}''\\
    % & & P134 & ``\textit{Giving advice for how to solve interpersonal issues based on available academic literature}''\\
    \texttt{Personal finance} & Q6 & P184 & ``\textit{Assist with budgeting and finances for people who struggle with budgeting}''\\
    \texttt{Personal life productivity} & Q3 & P26 & ``\textit{Provide a schedule to accomplish everything I want to get done today or this week}''\\ 
    \texttt{Accessibility marginalized}$^{*}$ & Q6 & P184 & ``\textit{Make technology more accessible to those with limited understanding or disabilities}''\\
    % \hline
    % \multicolumn{4}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\emph{Societal applications}}}\\
    % \hline
    % \texttt{Society} & Q6 & P67 & ``\textit{Propose ways to make education more affordable for all}''\\
    % & & P80 & ``\textit{Help solve racism}''\\
    % & & P107 & ``\textit{Finding solutions to climate change}''\\
    % & & P151 & ``\textit{Preventing future pandemics}''\\
    % & Q7 & P13 & ``\textit{Helping corporations get out of the boxed idea of the bottom line and become stewards to this planet as it was meant to be. And they do want it, just don't know how.}''\\
    % & & P28 & ``\textit{Predictive models that improve health and environment challenges.}''\\
    % & & P61 & ``\textit{the think tank group where Tech-X 10 would contribute equally with other members to help solve, for example, world hunger issues.}''\\
    \bottomrule
    \end{tabular}
    \caption{Examples of personal life applications, items that were coded with \texttt{everyday life assistance}, \texttt{everyday task automation}, etc., along with their additional characteristic codes. Code condensed due to space marked with ($*$).}
    \label{tab:personal-life-apps}
\end{table*}

==> content/tables-old/Q3-Q6-table.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{l|c|ll|l|c|ll}
    \toprule
        Theme & \makecell{Q3 (\%)\\\textit{N=1032}} & \multicolumn{2}{l|}{Code (\%)} & Theme & \makecell{Q6 (\%)\\\textit{N=992}} & \multicolumn{2}{l}{Code (\%)} \\
        \hline
        \multirow{3}{*}{domain} & \multirow{3}{*}{55.0} & artistic-expression & 24.3 & \multirow{3}{*}{domain} & \multirow{3}{*}{63.2} & medical & 16.6 \\
        & & education & 20.3 & & & education & 15.3\\
        && translation & 14.6& && research & 13.4\\
        \hline
        \multirow{2}{*}{personal life} & \multirow{2}{*}{45.7} & everyday-task-automation & 55.5 & \multirow{2}{*}{support type} & \multirow{2}{*}{39.3} & efficient-data-analysis & 44.4\\
        & & everyday-life-assistance & 39.0 & & & professional-consulting-service & 16.2 \\
        \hline
        \multirow{2}{*}{support type} & \multirow{2}{*}{39.0} & efficient-data-analysis & 22.9 & \multirow{2}{*}{personal life} & \multirow{2}{*}{39.2} & everyday-task-automation  & 56.3\\
        & & writing-assistance & 29.6 & & & everyday-life-assistance & 39.8\\
        \hline
        \multirow{2}{*}{goal of the use case} & \multirow{2}{*}{26.5} & creativity & 46.9 & \multirow{2}{*}{goal of the use case} & \multirow{2}{*}{25.9}  & personal-life-productivity & 23.3\\
        & & personal-life-productivity & 33.3 & & & creativity & 17.9\\
        \hline
        \multirow{2}{*}{work} & \multirow{2}{*}{5.2} & workplace-productivity & 85.2 & \multirow{2}{*}{society} & \multirow{2}{*}{8.7} & \multirow{2}{*}{societal-issues} & \multirow{2}{*}{100.0} \\
        & & human-labor-replacement & 14.8 & & & \\
        \hline
        \multirow{2}{*}{other} & \multirow{2}{*}{0.8} & \multirow{2}{*}{new-code} & \multirow{2}{*}{100.0} & \multirow{2}{*}{work} & \multirow{2}{*}{6.8} & human-labor-replacement & 70.6\\
        & & & & & & workplace-productivity & 36.8\\
        \hline
        society & 0.3 & societal-issues & 100.0 & other & 2.2 & new-code & 90.9 \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:q3-q6-theme-code-dist}
\end{table*}

==> content/tables-old/Q3-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q3 (\%)\\\textit{N=1032}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{55.0} & \texttt{artistic-expression} & 24.3 & \textit{``Make abstract art with my dog’s picture''} (P13)\\
        & & \texttt{education} & 20.3 & \textit{``Helping to teach coding''} (P213)\\
        & & \texttt{translation} & 14.6 & \textit{``Translations while traveling''} (P292)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{45.7} & \texttt{everyday-task-automation} & 55.5 & \textit{``Summarizing important email content into a list''} (P293)\\
        & & \texttt{everyday-life-assistance} & 39.0 & \textit{``Assisting with the layout for a fish tank''} (P130)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{39.0} & \texttt{writing-assistance} & 29.6 & \textit{``Adapting resumes to different job postings''} (P146)\\
        & & \texttt{efficient-data-analysis} & 22.9 & \textit{``Compiling obscure sports statistics''} (P127)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{26.5} & \texttt{creativity} & 46.9 & \textit{``Generating ideas and menus for parties''} (P80)\\
        & & \texttt{personal-life-productivity} & 33.3 & \textit{``Assisting with managing time spent on activities''} (P100)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{5.2} & \texttt{workplace-productivity} & 85.2 & \textit{``Proofreading policy proposals at work''} (P126)\\
        & & \texttt{human-labor-replacement} & 14.8 & \textit{``Automating tasks related to customer service''} (P84)\\
        \hline
        \textsc{other} & 0.8 & new-code & 100.0 & \textit{``Generate survey answers''} (P)\\
        \hline
        \textsc{society} & 0.3 & \texttt{societal-issues} & 100.0 & \textit{``Helping understand the dynamics of financial imperialism''} (P259)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q3-theme}
\end{table*}

==> content/tables-old/Q6-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q6 (\%)\\\textit{N=992}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{63.2} & \texttt{medical} & 16.6  & \textit{``Automating medical research''} (P54)\\
        & & \texttt{education} & 15.3 & \textit{``Acting as a personal tutor''} (P105)\\
        && \texttt{research} & 13.4 & \textit{``Revolutionize scientific research''} (P203)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{39.3} & \texttt{efficient-data-analysis} & 44.4 & \textit{``Assist in personalized medicine by analyzing genetic data, medical histories, and current research ...''} (P242)\\ 
        & & \texttt{professional-consulting-service} & 16.2  & \textit{``Act as a financial advisor''} (P103)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{39.2} & \texttt{everyday-task-automation}  & 56.3 & \textit{``Drive to any location hands-off''} (P172)\\
        & & \texttt{everyday-life-assistance} & 39.8 & \textit{``Acting as an advanced personal assistant''} (P213)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{25.9}  & \texttt{personal-life-productivity} & 23.3 & \textit{``Create plans to help achieve goals''} (P247)\\
        & & \texttt{creativity} & 17.9 & \textit{``Creating unique entertainment options that cater to individuals and evolve with them over time''} (P265)\\
        \hline
        \textsc{society} & 8.7 & \texttt{societal-issues} & 100.0 & \textit{``Assisting with or solving climate change issues''} (P262)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{6.8} & \texttt{human-labor-replacement} & 70.6 & \textit{``Replacing humans in customer interaction jobs''} (P282)\\
        & & \texttt{workplace-productivity} & 36.8 & \textit{``Generate job reports that would take a human hours to do''} (P86)\\
        \textsc{other} & 2.2 & \texttt{new-code} & 90.9 & \textit{``Find a way for the AI to destroy its own AI self''} (P25)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q6-theme}
\end{table*}

==> content/tables-old/Q7-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q7 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{67.8} & \texttt{medical} & 20.5 & \textit{``The task that I think Tech-X/Tech-X 10 would most dramatically change would be in personalized healthcare.''} (P85)\\
        & & \texttt{education} & 15.5 & \textit{``teaching me how to code in different languages efficiently and quickly''} (P104)\\
        & & \texttt{research} & 15.5 & \textit{``Solve difficult questions and do most of my tedious researches''} (P278)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{40.7} & \texttt{efficient-data-analysis} & 46.7 & \textit{``I think that Tech-X10 will most drastically change the way that we can consume data, and information based on it's ability to understand large amounts of data in a very short time frame. ''} (P174)\\
        & & \texttt{professional-consulting-service} & 19.2 & \textit{``Mental Health diagnosis and intervention. I believe Tech-X would really make a positive impact in this area, especially since, mental health professionals often gets overwhelmed with their work. Tech-X can serve as an assistant, in many ways''} (P203)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{33.6} & \texttt{personal-life-productivity} & 30.3 & \textit{``Inventing productive schedules to help improve my creative work, and being able to have casual conversations.''} (P123)\\
        & &  \texttt{creativity} & 19.2 & \textit{``Creating advertisements''} (P227)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{29.5} & \texttt{everyday-task-automation} & 48.3 & \textit{``Helping automatically complete taxes and pick out the right insurance for the best price.''} (P262)\\
        & & \texttt{everyday-life-assistance} & 47.1 & \textit{``assisting me with planning meal ideas that meet my family's dietary needs and restrictions.  This would take so much weight off my mental plate.''} (P249)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{10.8} & \texttt{human-labor-replacement} & 75 & \textit{``the need for human experts in most if not all fields.''} (P88)\\
        & & \texttt{workplace-productivity} & 37.5 & \textit{``It would eliminate the need for simple task to require humans to do repetitive tasks like excel and excel would instead give humans more time for meaningful tasks''} (P98)\\
        \hline
        \textsc{society} & 9.5 & \texttt{societal-issues} & 100 & \textit{``Predictive models that improve health and environment challenges.''} (P28)\\
        \hline
        \textsc{other} & 4.4 & \texttt{new-code} & 84.6 & \textit{``the aggregated audio books.''} (P35)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q7-theme}
\end{table*}

==> content/tables-old/Q8-table.tex <==
\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.23\linewidth}|p{0.71\linewidth}|p{0.1\linewidth}}
    \toprule
        & & \hfil \textbf{\% responses} \\
        \textbf{Code} & \textbf{Quote \& Scale of Impact (Q10)} & \hfil \textbf{Q8} \\
        & & \hfil $295\times$ \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Reinvest human capital}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.13$\pm$1.86} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{52.5\%} \\
        \hline
        \texttt{Personal life efficiency} &  \textit{``Save time, effort, and energy...[and] allow a layperson to accomplish this task.''} (P19) & \hfil 35.6\% \\
        \texttt{Personal growth} &  \hangindent=1em \textit{``Since it's data driven, individual performances will be vigorously assessed and suggest ways by which an individual can improve.''} (P47) & \hfil 16.9\% \\
        \texttt{Reduce mundane work} & \hangindent=1em \textit{``I would be able to focus on relationships and team building versus menial manager tasks that AI could complete for me.''} (P157) & \hfil 13.2\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Economic gain}}}  & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.38$\pm$1.75} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{43.7\%} \\
        \hline
        \texttt{General efficiency} & \hangindent=1em \textit{``Companies will not need to have as many employees...because they'll be able to automate much of the workload...which will increase company profits.''} (P209) & \hfil 31.5\% \\
        \texttt{Financial gain} & \textit{``It will save cost of different diagnostic tests.''} (P211) & \hfil 17.6\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Resource accessibility}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.58$\pm$1.62} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{35.9\%} \\
        \hline
        \texttt{Information accessibility} & \hangindent=1em \textit{``People need quick and reliable answers because not a lot of people have time for themselves...[and] can't deeply engage in topics they encounter in daily life.''} (P53) & \hfil 18.0\% \\
        \texttt{Resource accessibility} & \textit{``It would give people more equity and assistance.''} (P99) & \hfil 15.6\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Improve societal issues}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.96$\pm$1.25} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{31.9\%} \\
        \hline
        \texttt{Improve medical care} &  \textit{``Health care would be cheaper (hopefully) and more accessible to everyone''} (P109) & \hfil 13.2\% \\
        \texttt{Scientific research innovation} &  \textit{``Research would be able to be done at a faster pace.''} (P159) & \hfil 11.2\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Reduce error}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.11$\pm$1.57} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{16.9\%} \\
        \hline
        \texttt{Less human error} & \textit{``It could remove certain human biases''} (P171) & \hfil 10.8\% \\
        \texttt{Information quality} & \textit{``It could quickly detect lies said by politicians.''} (P229) & \hfil 9.8\% \\
        \hline
        \multicolumn{2}{l|}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Improve quality of personal life}}\hspace{112pt}\textbf{6.50$\pm$1.50}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{15.3\%} \\
        \hline
        \texttt{Improve well-being \& health} &  \textit{``My family would have a healthier diet \& they would live better lives.''} (P238) & \hfil 10.2\% \\
        \texttt{Improve mental health} & \textit{``It would reduce the cases of mental illness in lonely people.''} (P96) & \hfil 5.4\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Improve quality of social life}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{6.76$\pm$1.17} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{8.1\%} \\
        \hline
        \texttt{Better communication} & \textit{``People would be able to communicate in different languages in real-time.''} (P176) & \hfil 5.4\% \\
        \texttt{Social interaction} & \hangindent=1em \textit{``It would help me navigate through various social situations and problems, thus improving my social life.''} (P200) & \hfil 2.0\% \\
        \hline
        \multicolumn{1}{l}{\cellcolor[rgb]{ .921,  .921, .921}\textbf{\textsc{Other}}} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.25$\pm$2.17} & \cellcolor[rgb]{ .921,  .921, .921} \hfil \textbf{5.4\%} \\
        \hline
        \texttt{New code} &  \textit{``Help others with problems''} (P232) & \hfil 2.7\% \\
        \bottomrule
    \end{tabular}}
    \caption{Benefits of developing (Q8): Percentage of occurrence for \textsc{theme} with scale of impact (Q10) and corresponding top few most frequent \texttt{codes} with representative quotes.}
    \label{tab:q8-theme}
\end{table*}

% \begin{table}[htpb]
%     \centering
%     \footnotesize
%     \begin{tabularx}{\textwidth}{l|c|ll|X}
%     \toprule
%         Theme & \makecell{Q8 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
%         \hline
%         \multirow{3}{*}{\textsc{reinvest human capital}} & \multirow{3}{*}{52.5} & \texttt{personal-life-efficiency} & 67.7 & \textit{``It would save time effort and energy. It would also allow a layperson to accomplish this task.''} (P19)\\
%          & & \texttt{personal-growth} & 32.3 & \textit{``since its data driven, individual performances will be vigorously assessed and suggest ways by which an individual can improve''} (P47)\\
%          & & \texttt{reduce-mundane-work} & 25.2 & \textit{``I feel I would be able to focus on relationships and team building versus menial manager tasks that AI could complete for me.''} (P157)\\
%         \hline
%         \multirow{2}{*}{\textsc{economic gain}} & \multirow{2}{*}{43.7} & \texttt{general-efficiency} & 72.1 & \textit{``companies will not need to have as many employees in high salary positions because they'll be able to automate much of the workload; this will enable companies to considerably reduce salaries and overhead which will increase company profits.''} (P209)\\
%          & & \texttt{financial-gain} & 40.3 & \textit{``It will save cost of different diagonistic test. And also it will save life by ensuring that the right treatment is done''} (P211)\\
%         \hline
%         \multirow{2}{*}{\textsc{resource accessibility}} & \multirow{2}{*}{35.9} & \texttt{information-accessibility} & 50 & \textit{``People need quick and reliable answers because not a lot of people have time for themselves or the topic of the question they asked and cant deeply engage in topics they encounter in daily life.''} (P53)\\
%          & & \texttt{resource-accessibility} & 43.4 & \textit{``It would give people more equity and assistance.''} (P99)\\
%         \hline
%         \multirow{2}{*}{\textsc{improve societal issues}} & \multirow{2}{*}{31.9} & \texttt{improve-medical-care} & 41.5 & \textit{``Health care would be cheaper (hopefully) and more accessible to everyone''} (P109)\\
%          & & \texttt{scientific-research-innovation} & 35.1 & \textit{``Research would be able to be done at a faster pace.''} (P159)\\
%         \hline
%         \multirow{2}{*}{\textsc{reduce error}} & \multirow{2}{*}{16.9} & \texttt{less-human-error} & 64.0 & \textit{``it could remove certain human biases and provide excellent medical care''} (P171)\\
%          & & \texttt{information-quality} & 58.0 & \textit{``It could quickly detect lies said by politicians.''} (P229)\\
%         \hline
%         \multirow{2}{*}{\textsc{improve quality of personal life}} & \multirow{2}{*}{15.3} & \texttt{improve-well-being-health} & 66.7 & \textit{``my family would have a healthier diet \& they would live better lives.''} (P238)\\
%          & & \texttt{improve-mental-health} & 35.6 & \textit{``it would reduce the cases of mental illness in lonely people.''} (P96)\\
%         \hline
%         \multirow{2}{*}{\textsc{improve quality of social life}} & \multirow{2}{*}{8.1} & \texttt{better-communication} & 66.7 & \textit{``People would be able to communicate in different languages in real-time.''} (P176)\\
%          & & \texttt{social-interaction} & 25 & \textit{``it would help me navigate through various social situations and problems, thus improving my social life and probably teaching me a few things along the way.''} (P200)\\
%         \hline
%         other & 5.4 & \texttt{new-code} & 50 & \textit{``Help others with problems''} (P232)\\
%         \bottomrule
%     \end{tabularx}
%     \caption{Benefits of developing the application. Themes and corresponding codes with high frequencies of mentions and example quotes that were annotated with the code.}
%     \label{tab:q8-theme}
% \end{table}

==> content/tables/Q11-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q11 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{social and psychological effect}} & \multirow{3}{*}{35.3} & \texttt{manipulate-people} & 36.5 & \textit{``People would lose control potentially over important data, ideas, ...''} (P113)\\
         &  & \texttt{misinformation} & 35.6 & \textit{``It could give false information and confuse people as to where they don't know which source of information to trust''} (P126)\\
         &  & \texttt{mental-harm} & 34.6 & \textit{``People wanting to commit suicide maybe...''} (P67)\\
         \hline
        \multirow{2}{*}{\textsc{economic impact}} & \multirow{2}{*}{32.5} & \texttt{financial-disturbance} & 50 & \textit{``People would lose jobs and incomes''} (P93)\\
         &  & \texttt{economic-disturbance} & 39.6 & \textit{``Shortage in suppliers or a raise in costs''} (P131)\\
         \hline
        \multirow{2}{*}{\textsc{safety and security risk}} & \multirow{2}{*}{21.7} & \texttt{data-security-privacy-risk} & 48.4 & \textit{``Breach in privacy...''} (P179)\\
         &  & \texttt{extinction} & 26.6 & \textit{``human race eliminated by machines''} (P220)\\
         \hline
        \multirow{2}{*}{\textsc{physical effect}} & \multirow{2}{*}{16.9} & \texttt{physical-harm} & 76 & \textit{``Someone might fall very ill or even die''} (P246)\\
         &  & \texttt{negative-health-wellbeing} & 20 & \textit{``people would become more unhealthy''} (P175)\\
         \hline
        \multirow{2}{*}{\textsc{quality and reliability issues of AI}} & \multirow{2}{*}{15.9} & \texttt{incorrect-ai-output} & 61.7 & \textit{``people might be misdiagnosed and take action based on that''} (P264)\\
         &  & \texttt{distrust-ai} & 31.9 & \textit{``People would lose trust in technology''} (P72)\\
         \hline
        \multirow{2}{*}{\textsc{impeding human development and learning}} & \multirow{2}{*}{12.9} & \texttt{overreliance} & 73.7 & \textit{``it could steer people into a cult like dependency on AI as a blindly trusted leader.''} (P88)\\
         &  & \texttt{impede-learning} & 28.9 & \textit{``Diminished capacity for original ideas, maybe even critical thinking''} (P221)\\
         \hline
        \multirow{2}{*}{\textsc{reducing quality and reliability of society}} & \multirow{2}{*}{12.2} & \texttt{distrust-institution} & 47.2 & \textit{``If widespread, it could cause a financial meltdown and a complete lack of trust in companies. ''} (P255)\\
         &  & \texttt{legal-issues} & 25 & \textit{``possible biological agents or increased lawsuits.''} (P95)\\
         \hline
        \multirow{2}{*}{\textsc{general harm}} & \multirow{2}{*}{6.8} & \texttt{general-harm} & 70 & \textit{``More people would be hurt''} (P105)\\
         &  & \texttt{range} & 30 & \textit{``A select few suffering more than others.''} (P108)\\
         \hline
        \multirow{2}{*}{\textsc{other}} & \multirow{2}{*}{4.4} & \texttt{na} & 53.8 & \textit{``many things''} (P216)\\
         &  & \texttt{no-harm} & 38.5 & \textit{``I can’t think of any''} (P242)\\
         \hline
        \multirow{2}{*}{\textsc{reducing progress}} & \multirow{2}{*}{2.0} & \texttt{environmental-harm} & 66.7 & \textit{``Climate change could be made even worse.''} (P140)\\
         &  & \texttt{hinder-science} & 33.3 & \textit{``It will destroy the integrity of scientific advancements''} (P276)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q11-theme}
\end{table*}

==> content/tables/Q14-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q14 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{economic impact}} & \multirow{2}{*}{33.6} & \texttt{financial-disturbance} & 61.6 & \textit{``Money wasted.''} (P8)\\
         &  & \texttt{economic-disturbance} & 29.3 & \textit{``impoverising the poor more.''} (P54)\\
         &  & \texttt{waste-resources-or-time} & 28.3 & \textit{``potentially leading to misguided decisions, wasted resources, and exacerbation of existing problems.''} (P250)\\
        \hline
        \multirow{2}{*}{\textsc{physical effect}} & 29.8 & \texttt{physical-harm} & 79.5 & \textit{``It could lead to serious injury  or death.''} (P215)\\
         &  & \texttt{negative-health-wellbeing} & 28.4 & \textit{``Poorer health''} (P242)\\
        \hline
        \multirow{2}{*}{\textsc{social and psychological effect}} & 26.4 & \texttt{misinformation} & 41 & \textit{``Action would be taken on invalid info with potential harm''} (P244)\\
         &  & \texttt{mental-harm} & 35.9 & \textit{``Loss of confidence and motivation: Repeated misunderstandings and failed interactions could lead to frustration and a reluctance to engage in further language learning.''} (P280)\\
         &  & \texttt{social-isolation} & 16.7 & \textit{``It would harm social relationships. Not necessarily ending them, but maybe lead to ostracism or loss of trust.''} (P200)\\
        \hline
        \multirow{2}{*}{\textsc{quality and reliability issues of AI}} & 24.1 & \texttt{incorrect-ai-output} & 56.3 & \textit{``It depends on the situation, but for example, providing incorrect or incomplete medical diagnostics''} (P221)\\
         &  & \texttt{distrust-ai} & 23.9 & \textit{``People would start protesting and would try to ban this AI.''} (P50)\\
        \hline
        \multirow{2}{*}{\textsc{impeding human development and learning}} & 12.5 & \texttt{overreliance} & 54.1 & \textit{``They will not learn to do anything on their own''} (P274)\\
         &  & \texttt{hinder-career} & 32.4 & \textit{``The reputation of the developers would be ruined''} (P125)\\
        \hline
        \multirow{2}{*}{\textsc{general harm}} & 11.5 & \texttt{general-harm} & 88.2 & \textit{``I think providing incorrect information could generally just make people's lives harder.''} (P166)\\
         &  & \texttt{range} & 14.7 & \textit{``Could cause anything from minor issues to loss of life''} (P271)\\
        \hline
        \multirow{2}{*}{\textsc{reducing quality and reliability of society}} & 9.2 & \texttt{distrust-institution} & 59.3 & \textit{``The negative impact would be loss of business and decreased trust in the medical professionals...''} (P)\\
         &  & \texttt{legal-issues} & 44.4 & \textit{``It would lead to injuries and potential legal issues.''} (P41)\\
        \hline
        \multirow{2}{*}{\textsc{safety and security risk}} & 7.8 & \texttt{data-security-privacy-risk} & 39.1 & \textit{``It could be anything from software failure to compromising users private data''} (P235)\\
         &  & \texttt{aid-criminal} & 34.8 & \textit{``It will lead to theft''} (P275)\\
        \hline
      \textsc{other} & 7.1 & \texttt{no-harm} & 52.4 & \textit{``none''} (P)\\
        \hline
        \multirow{2}{*}{\textsc{reducing progress}} & 4.7 & \texttt{hinder-science} & 64.3 & \textit{``Delay scientific advancement and progress''} (P276)\\
         &  & \texttt{environmental-harm} & 35.7 & \textit{``it could negatively impact fighting climate change''} (P23)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q14-theme}
\end{table*}

==> content/tables/Q3-Q6-table.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{l|c|ll|l|c|ll}
    \toprule
        Theme & \makecell{Q3 (\%)\\\textit{N=1032}} & \multicolumn{2}{l|}{Code (\%)} & Theme & \makecell{Q6 (\%)\\\textit{N=992}} & \multicolumn{2}{l}{Code (\%)} \\
        \hline
        \multirow{3}{*}{domain} & \multirow{3}{*}{55.0} & artistic-expression & 24.3 & \multirow{3}{*}{domain} & \multirow{3}{*}{63.2} & medical & 16.6 \\
        & & education & 20.3 & & & education & 15.3\\
        && translation & 14.6& && research & 13.4\\
        \hline
        \multirow{2}{*}{personal life} & \multirow{2}{*}{45.7} & everyday-task-automation & 55.5 & \multirow{2}{*}{support type} & \multirow{2}{*}{39.3} & efficient-data-analysis & 44.4\\
        & & everyday-life-assistance & 39.0 & & & professional-consulting-service & 16.2 \\
        \hline
        \multirow{2}{*}{support type} & \multirow{2}{*}{39.0} & efficient-data-analysis & 22.9 & \multirow{2}{*}{personal life} & \multirow{2}{*}{39.2} & everyday-task-automation  & 56.3\\
        & & writing-assistance & 29.6 & & & everyday-life-assistance & 39.8\\
        \hline
        \multirow{2}{*}{goal of the use case} & \multirow{2}{*}{26.5} & creativity & 46.9 & \multirow{2}{*}{goal of the use case} & \multirow{2}{*}{25.9}  & personal-life-productivity & 23.3\\
        & & personal-life-productivity & 33.3 & & & creativity & 17.9\\
        \hline
        \multirow{2}{*}{work} & \multirow{2}{*}{5.2} & workplace-productivity & 85.2 & \multirow{2}{*}{society} & \multirow{2}{*}{8.7} & \multirow{2}{*}{societal-issues} & \multirow{2}{*}{100.0} \\
        & & human-labor-replacement & 14.8 & & & \\
        \hline
        \multirow{2}{*}{other} & \multirow{2}{*}{0.8} & \multirow{2}{*}{new-code} & \multirow{2}{*}{100.0} & \multirow{2}{*}{work} & \multirow{2}{*}{6.8} & human-labor-replacement & 70.6\\
        & & & & & & workplace-productivity & 36.8\\
        \hline
        society & 0.3 & societal-issues & 100.0 & other & 2.2 & new-code & 90.9 \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:q3-q6-theme-code-dist}
\end{table*}

==> content/tables/Q3-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q3 (\%)\\\textit{N=1032}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{55.0} & \texttt{artistic-expression} & 24.3 & \textit{``Make abstract art with my dog’s picture''} (P13)\\
        & & \texttt{education} & 20.3 & \textit{``Helping to teach coding''} (P213)\\
        & & \texttt{translation} & 14.6 & \textit{``Translations while traveling''} (P292)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{45.7} & \texttt{everyday-task-automation} & 55.5 & \textit{``Summarizing important email content into a list''} (P293)\\
        & & \texttt{everyday-life-assistance} & 39.0 & \textit{``Assisting with the layout for a fish tank''} (P130)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{39.0} & \texttt{writing-assistance} & 29.6 & \textit{``Adapting resumes to different job postings''} (P146)\\
        & & \texttt{efficient-data-analysis} & 22.9 & \textit{``Compiling obscure sports statistics''} (P127)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{26.5} & \texttt{creativity} & 46.9 & \textit{``Generating ideas and menus for parties''} (P80)\\
        & & \texttt{personal-life-productivity} & 33.3 & \textit{``Assisting with managing time spent on activities''} (P100)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{5.2} & \texttt{workplace-productivity} & 85.2 & \textit{``Proofreading policy proposals at work''} (P126)\\
        & & \texttt{human-labor-replacement} & 14.8 & \textit{``Automating tasks related to customer service''} (P84)\\
        \hline
        \textsc{other} & 0.8 & new-code & 100.0 & \textit{``Generate survey answers''} (P)\\
        \hline
        \textsc{society} & 0.3 & \texttt{societal-issues} & 100.0 & \textit{``Helping understand the dynamics of financial imperialism''} (P259)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q3-theme}
\end{table*}

==> content/tables/Q6-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q6 (\%)\\\textit{N=992}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{63.2} & \texttt{medical} & 16.6  & \textit{``Automating medical research''} (P54)\\
        & & \texttt{education} & 15.3 & \textit{``Acting as a personal tutor''} (P105)\\
        && \texttt{research} & 13.4 & \textit{``Revolutionize scientific research''} (P203)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{39.3} & \texttt{efficient-data-analysis} & 44.4 & \textit{``Assist in personalized medicine by analyzing genetic data, medical histories, and current research ...''} (P242)\\ 
        & & \texttt{professional-consulting-service} & 16.2  & \textit{``Act as a financial advisor''} (P103)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{39.2} & \texttt{everyday-task-automation}  & 56.3 & \textit{``Drive to any location hands-off''} (P172)\\
        & & \texttt{everyday-life-assistance} & 39.8 & \textit{``Acting as an advanced personal assistant''} (P213)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{25.9}  & \texttt{personal-life-productivity} & 23.3 & \textit{``Create plans to help achieve goals''} (P247)\\
        & & \texttt{creativity} & 17.9 & \textit{``Creating unique entertainment options that cater to individuals and evolve with them over time''} (P265)\\
        \hline
        \textsc{society} & 8.7 & \texttt{societal-issues} & 100.0 & \textit{``Assisting with or solving climate change issues''} (P262)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{6.8} & \texttt{human-labor-replacement} & 70.6 & \textit{``Replacing humans in customer interaction jobs''} (P282)\\
        & & \texttt{workplace-productivity} & 36.8 & \textit{``Generate job reports that would take a human hours to do''} (P86)\\
        \textsc{other} & 2.2 & \texttt{new-code} & 90.9 & \textit{``Find a way for the AI to destroy its own AI self''} (P25)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q6-theme}
\end{table*}

==> content/tables/Q7-table.tex <==
\begin{table*}[htpb]
    \centering
    \footnotesize
    \begin{tabularx}{\textwidth}{l|c|ll|X}
    \toprule
        Theme & \makecell{Q7 (\%)\\\textit{N=295}} & \multicolumn{2}{l|}{Code (\%)} & Quote\\
        \hline
        \multirow{3}{*}{\textsc{domain}} & \multirow{3}{*}{67.8} & \texttt{medical} & 20.5 & \textit{``The task that I think Tech-X/Tech-X 10 would most dramatically change would be in personalized healthcare.''} (P85)\\
        & & \texttt{education} & 15.5 & \textit{``teaching me how to code in different languages efficiently and quickly''} (P104)\\
        & & \texttt{research} & 15.5 & \textit{``Solve difficult questions and do most of my tedious researches''} (P278)\\
        \hline
        \multirow{2}{*}{\textsc{support type}} & \multirow{2}{*}{40.7} & \texttt{efficient-data-analysis} & 46.7 & \textit{``I think that Tech-X10 will most drastically change the way that we can consume data, and information based on it's ability to understand large amounts of data in a very short time frame. ''} (P174)\\
        & & \texttt{professional-consulting-service} & 19.2 & \textit{``Mental Health diagnosis and intervention. I believe Tech-X would really make a positive impact in this area, especially since, mental health professionals often gets overwhelmed with their work. Tech-X can serve as an assistant, in many ways''} (P203)\\
        \hline
        \multirow{2}{*}{\textsc{goal of the use case}} & \multirow{2}{*}{33.6} & \texttt{personal-life-productivity} & 30.3 & \textit{``Inventing productive schedules to help improve my creative work, and being able to have casual conversations.''} (P123)\\
        & &  \texttt{creativity} & 19.2 & \textit{``Creating advertisements''} (P227)\\
        \hline
        \multirow{2}{*}{\textsc{personal life}} & \multirow{2}{*}{29.5} & \texttt{everyday-task-automation} & 48.3 & \textit{``Helping automatically complete taxes and pick out the right insurance for the best price.''} (P262)\\
        & & \texttt{everyday-life-assistance} & 47.1 & \textit{``assisting me with planning meal ideas that meet my family's dietary needs and restrictions.  This would take so much weight off my mental plate.''} (P249)\\
        \hline
        \multirow{2}{*}{\textsc{work}} & \multirow{2}{*}{10.8} & \texttt{human-labor-replacement} & 75 & \textit{``the need for human experts in most if not all fields.''} (P88)\\
        & & \texttt{workplace-productivity} & 37.5 & \textit{``It would eliminate the need for simple task to require humans to do repetitive tasks like excel and excel would instead give humans more time for meaningful tasks''} (P98)\\
        \hline
        \textsc{society} & 9.5 & \texttt{societal-issues} & 100 & \textit{``Predictive models that improve health and environment challenges.''} (P28)\\
        \hline
        \textsc{other} & 4.4 & \texttt{new-code} & 84.6 & \textit{``the aggregated audio books.''} (P35)\\
        \bottomrule
    \end{tabularx}
    \caption{Caption}
    \label{tab:q7-theme}
\end{table*}

==> content/tables/hb-dev-scale.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{lll|ll}
    \toprule
        \multicolumn{3}{l|}{\textbf{Harms of Developing}} & \multicolumn{2}{l}{\textbf{Benefits of Developing}} \\
        \hline
        \cellcolor[rgb]{ .921,  .921, .921}\textbf{Themes (Q11 \& Q14)} & \cellcolor[rgb]{ .921,  .921, .921}\textbf{Scale (Q13)} & \cellcolor[rgb]{ .921,  .921, .921}\textbf{Scale (Q16)} & \cellcolor[rgb]{ .921,  .921, .921}\textbf{Themes (Q8)} & \cellcolor[rgb]{ .921,  .921, .921}\textbf{Scale (Q10)} \\
        \hline
        \textsc{Physical effect} & 6.70$\pm$1.40 & 6.28$\pm$1.59 & \textsc{Improve quality of social life} & 6.76$\pm$1.17\\
        \textsc{Safety and security risk} & 6.32$\pm$1.57 & 6.10$\pm$1.60 & \textsc{Improve quality of personal life} & 6.50$\pm$1.50\\
        \textsc{General harm} & 5.95$\pm$2.25 & 5.97$\pm$1.94 & \textsc{Reduce error} & 6.11$\pm$1.57\\
        \textsc{Social and psychological effect} & 5.82$\pm$1.94 & 5.29$\pm$2.05 & \textsc{Resource accessibility} & 5.58$\pm$1.62\\
        \textsc{Reducing quality and reliability of society} & 5.70$\pm$2.01 & 5.48$\pm$2.09 & \textsc{Economic gain} & 5.38$\pm$1.75\\
        \textsc{Economic impact} & 5.39$\pm$1.70 & 4.63$\pm$1.75 & \textsc{Reinvest human capital} & 5.13$\pm$1.86 \\
        \textsc{Quality and reliability issues of AI} & 5.16$\pm$1.76 & 5.43$\pm$2.12 & \textsc{Other} & 5.25$\pm$2.17\\
        \textsc{Impeding human development and learning} & 4.41$\pm$1.80 & 4.42$\pm$2.10 & & \\
        \textsc{Other} & 3.30$\pm$3.22 & 4.28$\pm$2.83 & & \\
        \hline
        Total & 5.47$\pm$2.00 & 5.21$\pm$2.08 & Total & 5.68$\pm$1.85\\
        \bottomrule
    \end{tabular}
    \caption{Mean and standard deviation of scale of benefit and harm of developing the application aggregated by themes.}
    \label{tab:hb-dev-scale}
\end{table*}

==> content/tables/hb-not-dev-scale.tex <==
\begin{table*}[]
    \centering
    \footnotesize
    \begin{tabular}{ll|ll}
        \toprule
        \multicolumn{2}{l|}{\textbf{Harms of Not Developing}} & \multicolumn{2}{l}{\textbf{Benefits of Not Developing}}\\
        \hline
        \cellcolor[rgb]{.921, .921, .921}\textbf{Themes (Q17)} & \cellcolor[rgb]{.921, .921, .921}\textbf{Scale (Q19)} & \cellcolor[rgb]{.921, .921, .921}\textbf{Themes (Q20)} & \cellcolor[rgb]{.921, .921, .921}\textbf{Scale (Q22)}\\
        \hline
        \textsc{Physical effect} & 5.14$\pm$2.62 & \textsc{Beneficial side effects of not using ai} & 4.75$\pm$2.71 \\
        \textsc{Less progress in solving societal issues} & 4.78$\pm$2.19 & \textsc{Human growth and potential} & 3.95$\pm$2.08 \\
        \textsc{Less innovation} & 4.64$\pm$2.08 & \textsc{Less bad ai usage} & 3.66$\pm$2.41 \\
        \textsc{Limited to human capabilities} & 4.39$\pm$1.64 & \textsc{Economic impact / security} & 3.54$\pm$2.23\\
        \textsc{Lose information and accessibility to resources} & 4.14$\pm$2.04 & \textsc{Increase transparency, control, and reliability} & 3.34$\pm$2.06 \\
        \textsc{Social and psychological effect} & 4.07$\pm$2.40 & \textsc{No changes} & 3.26$\pm$2.33\\
        \textsc{Economic and business impact} & 3.70$\pm$2.27 & \textsc{Other} & 3.05$\pm$2.79\\
        \textsc{Limiting human potential} & 3.56$\pm$2.12 & & \\
        \textsc{Other} & 2.73$\pm$2.59 & & \\
        \hline
        Total & 3.68$\pm$2.32 & Total & 3.53$\pm$2.35\\
        \bottomrule
    \end{tabular}
    \caption{Mean and standard deviation of scale of benefits and harms of not developing the application aggregated by themes.}
    \label{tab:hb-not-dev-scale}
\end{table*}
